Sniff AI: Is My 'Spicy' Your 'Spicy'? Exploring LLM's Perceptual Alignment with Human Smell Experiences

Aligning AI with human intent is important, yet perceptual alignment-how AI interprets what we see, hear, or smell-remains underexplored. This work focuses on olfaction, human smell experiences. We conducted a user study with 40 participants to investigate how well AI can interpret human descriptions of scents. Participants performed "sniff and describe" interactive tasks, with our designed AI system attempting to guess what scent the participants were experiencing based on their descriptions. These tasks evaluated the Large Language Model's (LLMs) contextual understanding and representation of scent relationships within its internal states - high-dimensional embedding space. Both quantitative and qualitative methods were used to evaluate the AI system's performance. Results indicated limited perceptual alignment, with biases towards certain scents, like lemon and peppermint, and continued failing to identify others, like rosemary. We discuss these findings in light of human-AI alignment advancements, highlighting the limitations and opportunities for enhancing HCI systems with multisensory experience integration.

==> tables/ingredient.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{minipage}
\begin{table}[h]
\caption{Scent used in the study and their ingredients}
\label{tab:ingredients}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Families &
  Subfamilies &
  ID &
  Scent &
  CAS \tablefootnote{CAS number source websites: Chemical Substance Search (\url{https://www.echemportal.org/echemportal/substance-search}); Spectrum Chemical Home (\url{https://www.spectrumchemical.com/})} &
  Source of Ingredients \\ \midrule
 &
  Aromatic &
  1 &
  rosemary &
  8000-25-7 &
  Rosmarinus Officinalis leaf oil \\
 &
  Aromatic &
  2 &
  eucalyptus &
  84625-32-1 &
  Eucalptus Globulus leaf oil \\
Fresh &
  Citrus &
  3 &
  bergamot &
  8007-75-8 &
  Citrus Aurantium Bergamia peel oil \\
 &
  Fruity &
  4 &
  lemon &
  {\color[HTML]{242424} 8008-56-8} &
  Citrus Limon peel oil, Limonene, Citral \\
 &
  Green &
  5 &
  Peppermint &
  8006-90-4 &
  Mentha Arvensis oil \\ \midrule
 &
  Floral &
  6 &
  lavender &
  8000-28-0 &
  Lavandual Angustifolia oil, linalool, geraniol, lemonene, coumarin \\
 &
  Floral &
  7 &
  gardenia &
  {\color[HTML]{444444} 68916-47-2} &
  White flowers of the Gardenia jasminoides tree extracts \\
Floral &
  Soft Floral &
  8 &
  rose &
  8007-01-0 &
  \begin{tabular}[c]{@{}l@{}}Prinus Amygdalus Dulcius oil (sweet almond), Rosa Damanscena oil, \\ Tocopherol\end{tabular} \\
 &
  Floral Oriental &
  9 &
  jasmin &
  84776-64-7 &
  \begin{tabular}[c]{@{}l@{}}Prinus Amygdalus Dulcius oil (sweet almond), Jasminum Grandiflorum \\ flower extract, Tocopherol\end{tabular} \\
 &
  Floral Oriental &
  10 &
  geranium &
  8000-46-2 &
  \begin{tabular}[c]{@{}l@{}}Pelargonium graveolens flower oil, Cital, Geraniol, Linalool, \\ Citronellol, Limonene\end{tabular} \\ \midrule
 &
  Soft Oriental &
  11 &
  vanilla &
  8047-24-3 &
  \begin{tabular}[c]{@{}l@{}}Prinus Amygdalus Dulcius oil (sweet almond), \\ Vanilla Planifolia oil, Tocopherol\end{tabular} \\
 &
  Soft Oriental &
  12 &
  cardamom &
  {\color[HTML]{242424} 8000-66-6} &
  \begin{tabular}[c]{@{}l@{}}Prinus Amygdalus Dulcius oil (sweet almond), \\ Elettaria Cardamomum (seed) oil, Tocopherol\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Oriental\\ (amber)\end{tabular} &
  Oriental &
  13 &
  frankincense &
  \begin{tabular}[c]{@{}l@{}}8016-36-2/ \\ 89957-98-2\end{tabular} &
  Boswellia Carterii oil, limonene, Linalool \\
 &
  Woody Oriental &
  14 &
  sandalwood &
  {\color[HTML]{242424} 8006-87-9} &
  Santalum album tree bark \\
 &
  Woody Oriental &
  15 &
  patchouli &
  {\color[HTML]{242424} 8014-09-3} &
  Pogostemon Cablin (patchouli) Leaf oil \\ \midrule
 &
  Woods &
  16 &
  pine &
  {\color[HTML]{242424} 84012-35-1} &
  Pinus Sylvestris (Pine) oil \\
 &
  Woods &
  17 &
  cedarwood &
  {\color[HTML]{242424} 8000-27-9} &
  Juniperus Virginiana (cedarwood) oil, sunflower seed oil \\
Woody &
  Mossy Woods &
  18 &
  oakmoss &
  {\color[HTML]{242424} 9000-50-4} &
  lichen Evernia prunastri \\
 &
  Dry Woods &
  19 &
  black pepper &
  {\color[HTML]{242424} 8006-82-4} &
  Piper nigrum plant \\
 &
  Dry Woods &
  20 &
  cinnamon &
  {\color[HTML]{242424} 8015-91-6} &
  \begin{tabular}[c]{@{}l@{}}Cinnamomum Zetlanicum (Cinnamon) leaf oil, Benzyl Benzoate, \\ Cinnamyl Alcohol, Cinnamal, Eugenol, Linalool, Coumarin\end{tabular} \\ \bottomrule
\end{tabular}}
\end{table}
% \end{minipage}

==> tables/metrics.tex <==
% \usepackage{booktabs}

% (0 = "Not Similar at All
% 10 = "Completely Similar")


% \usepackage{booktabs}


\begin{table}
\centering
\caption{Overview of Evaluation Metrics}
\label{tab:eval_metrics}
\begin{tabular}{c|l|l}
\textbf{Metric}                                                & \multicolumn{1}{c|}{\textbf{Description}}                                                                                                                             & \multicolumn{1}{c}{\textbf{Measurement}}                                                                     \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}AI Success \\Rate\end{tabular}      & \begin{tabular}[c]{@{}l@{}}The proportion of correct scent predictions \\made by the AI in each task.\end{tabular}                                                    & Correct guesses / Total rounds per task                                                                       \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Validity \\Score\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Rating by participants of how accurately the AI's guesses \\reflect their scent descriptions,even when predictions incorrect.\end{tabular} & \begin{tabular}[c]{@{}l@{}}11-point scale~~(0 = "Not Valid at All\\10 = "Completely Valid")\end{tabular}      \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Similarity \\Score\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Participants' rating of the perceived similarity between the \\reference (AI's guessed) scent and the actual target scent.\end{tabular}    & \begin{tabular}[c]{@{}l@{}}11-point scale~ (0 = "Not Similar at All\\10 = "Completely Similar")\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Qualitative \\Insights\end{tabular} & \begin{tabular}[c]{@{}l@{}}Participant feedback on their interaction with the AI, including \\perceptions of its performance and applications.\end{tabular}           & Semi-structured interviews                                                                                   
\end{tabular}
\end{table}
